Equilibria of Fully Decentralized Learning in Networked Systems

Existing settings of decentralized learning either require players to have full information or the system to have certain special structure that may be hard to check and hinder their applicability to practical systems. To overcome this, we identify a structure that is simple to check for linear dynamical system, where each player learns in a fully decentralized fashion to minimize its cost. We first establish the existence of pure strategy Nash equilibria in the resulting noncooperative game. We then conjecture that the Nash equilibrium is unique provided that the system satisfies an additional requirement on its structure. We also introduce a decentralized mechanism based on projected gradient descent to have agents learn the Nash equilibrium. Simulations on a $5$-player game validate our results.

==> 05-conjecture.tex <==
%\textcolor{red}{To do: Give proof for 2by2 case}




% Inspired by~\cite{gadjov2018passivity}, we conduct decentralized gradient descent for each agent, which admits  a  gradient-based dynamics  for each player $i$
% \begin{align}\label{eq:gradient}
% \mathcal{P}_i: \quad \dot{k}_i=\left[-\nabla_i J_i\left(k_i,k_{-i}\right)\right]^+_{k_i} \quad \forall i \in \mathcal{I}\,,
% \end{align}
% where, $\forall \boldsymbol{\alpha}:=\left(\alpha_i(t), i \in \left[n\right] \right) \in \real^n$ and $\boldsymbol{\beta}:=\left(\beta_i(t), i \in \left[n\right] \right) \in \real^n$ the element-wise projection operator $\left[\boldsymbol{\alpha}\right]^+_{\boldsymbol{\beta}}$ defined by~\cite{mallada2017tac, you2021tac} 
% \begin{align}\label{eq:def_proj}
% \left[\boldsymbol{\alpha}\right]^+_\boldsymbol{\beta}&:=\left(\left[\alpha_i(t)\right]^+_{\beta_i(t)}, i \in \left[n\right] \right)\qquad\text{with}\qquad\left[\alpha_i(t)\right]^+_{\beta_i(t)}:=\!\begin{cases}
% 	\alpha_i &\!\!\textrm{if $\alpha_i>0$ or $\beta_i>0$}\\	0&\!\!\textrm{otherwise}\nonumber
% 	\end{cases}
% \end{align}
% ensures that $k_i$ remains nonnegative, i.e, $k_i\geq0$.
% \begin{thm}[Global asymptotic stability] The noncooperative game with each player adopts a projected gradient dynamics described by the closed-loop system in \textcolor{red}{()}{} converges globally asymptotically to the unique Nash equilibrium $(\mathbbold{0}_n,\boldsymbol{k}^\ast)$.

% \end{thm}
% \begin{proof}
% Consider the following quadratic Lyapunov function: 
% \begin{align}\label{eq:V}
%     V(\boldsymbol{x}, \boldsymbol{k}):=\dfrac{1}{2}\boldsymbol{x}^2+\dfrac{1}{2}\|\boldsymbol{k}-\boldsymbol{k}^\ast\|^2_2\,,
% \end{align}
% where $\|\cdot\|_2$ denotes the Euclidean norm.
% Then the derivative of $V(\boldsymbol{x}, \boldsymbol{k})$ along the trajectories of the closed-loop system is 
% \begin{align}\label{eq:Vdot}
%     \dot{V}(\boldsymbol{x}, \boldsymbol{k})&=\boldsymbol{x}^T\dot{\boldsymbol{x}}+\left(\boldsymbol{k}-\boldsymbol{k}^\ast\right)^T\dot{\boldsymbol{k}}\nonumber\\&=\boldsymbol{x}^T\left(\boldsymbol{A}-\boldsymbol{K}\right)\boldsymbol{x}+\left(\boldsymbol{k}-\boldsymbol{k}^\ast\right)^T \left[-g(\boldsymbol{k})\right]^+_\boldsymbol{k}\nonumber\\&\stackrel{\circled{1}}{\leq}0+\left(\boldsymbol{k}-\boldsymbol{k}^\ast\right)^T \left(-g(\boldsymbol{k})\right)\nonumber\\
%     &\stackrel{\circled{2}}{=}-\left(\boldsymbol{k}-\boldsymbol{k}^\ast\right)^T \left(g(\boldsymbol{k})-g(\boldsymbol{k}^\ast)\right)<0\,,\qquad\forall(\boldsymbol{x},\boldsymbol{k})\neq(\mathbbold{0}_n,\boldsymbol{k}^\ast)\,.
% \end{align}
% In \circled{1}, we use the Assumption~\ref{ass:sys} that $\boldsymbol{A}-\boldsymbol{K}\prec0$ and the non-expansive property of the projection operator, i.e., $\left(\boldsymbol{k}-\boldsymbol{k}^\ast\right)^T \left[-g(\boldsymbol{k})\right]^+_{\boldsymbol{k}}\leq\left(\boldsymbol{k}-\boldsymbol{k}^\ast\right)^T \left(-g(\boldsymbol{k})\right)$, due to the fact that the $i$th projection is active, i.e., $\left[-g_i(\boldsymbol{k})\right]^+_{k_i}=0$, only if both $-g_i(\boldsymbol{k}) \leq 0$ and $k_i \leq 0$, which still implies that $\left(k-k_i^\ast\right)\left[-g_i(\boldsymbol{k})\right]^+_{k_i} = 0 \leq \left(k-k_i^\ast\right)g_i(\boldsymbol{k})$ whenever $k_i^\ast\geq0$. In \circled{2}, the fact that $g(\boldsymbol{k}^\ast)=0$ and the strict monotonicity condition in Conjecture~\ref{conj:strict-mono} is used. Therefore, \eqref{eq:Vdot} together with the fact that $V(\boldsymbol{x}, \boldsymbol{k})$ in \eqref{eq:V} is radially unbounded implies that the game described by the closed-loop system converges globally asymptotically to the equilibrium point $(\mathbbold{0}_n,\boldsymbol{k}^\ast)$.\end{proof}

% or, $\mathcal{P}: \dot{k}=-F(k)$, the overall system of all the agents' dynamics stacked together.  Convergence of~\eqref{eq:gradient} is also guaranteed under strict (strong) monotonicity on the pseudogradient $F$~\cite{gadjov2018passivity}. 





% \begin{lem} The decentralized gradient-based updates converge to a unique Nash Equilibrium satisfies
% \begin{align}\label{eq:Nash}
%     \nabla_i J_i\left(k_i^*,k_{-i}^*\right)=0 \quad \forall i \in [n]
% \end{align}
% \end{lem}
% \begin{proof}
% From lemma [], $\mathcal{D}^i$ is a closed, bounded and convex subset of a finite-dimensional Euclidean space. 

% The strict convexity of $J_i\left(k_i,k_{-i}\right)$ gives $(k_i-k_i^\prime)^T(F(k_i)-F(k_i^\prime))>0 $ for all $i$. Hence, $(k-k')^T(F(k)-F(k'))>0, \forall k\neq k'$. 



% % From~\cite[Lemma 3]{scutari2014real}, the game has a unique Nash Equilibrium if the pseudo-gradient is strictly monotone, which is satisfied by the strict convexity of $J_i\left(k_i,k_{-i}\right)$ 
% \end{proof}



% Gradient-Based Update rule
% \begin{align}\label{eq:k-dyn}
%     \dot{k}_i=-\dfrac{\partial J_i(\boldsymbol{K})}{\partial k_i}=&-\ \rho_i k_i f_i(\boldsymbol{K})-\dfrac{\left(1+\rho_i k_i^2\right)}{2}\dfrac{\partial f_i(\boldsymbol{K})}{\partial k_i}\\
%     =&\ -\rho_i k_i f_i(\boldsymbol{K})+\dfrac{\left(1+\rho_i k_i^2\right)}{2}f^2_i(\boldsymbol{K})
% \end{align}
% From \eqref{eq:Ji}, we know  
% \begin{align}\label{eq:Ji-1}
%     J_i(\boldsymbol{K})=\dfrac{\left(1+\rho_i k_i^2\right)}{2} \boldsymbol{e}_i^T \left(\boldsymbol{K}-\boldsymbol{A}\right)^{-1}\boldsymbol{e}_i=\dfrac{\left(1+\rho_i k_i^2\right)}{2} f_i(\boldsymbol{K})\,.
% \end{align}
% Thus, 
% \begin{align}\label{eq:fi-Ji}
%     f_i(\boldsymbol{K})=\dfrac{2J_i(\boldsymbol{K})}{1+\rho_i k_i^2}\,.
% \end{align}
% Substituting \eqref{eq:fi-Ji} to \eqref{eq:k-dyn} yields
% \begin{align}
%     \dot{k}_i
%     =&\ -\rho_i k_i \dfrac{2J_i(\boldsymbol{K})}{1+\rho_i k_i^2}+\dfrac{\left(1+\rho_i k_i^2\right)}{2}\left(\dfrac{2J_i(\boldsymbol{K})}{1+\rho_i k_i^2}\right)^2\\=&\ -\rho_i k_i \dfrac{2J_i(\boldsymbol{K})}{1+\rho_i k_i^2}+\dfrac{2J_i^2(\boldsymbol{K})}{1+\rho_i k_i^2}=\dfrac{2J_i(\boldsymbol{K})}{1+\rho_i k_i^2}\left(J_i(\boldsymbol{K})-\rho_i k_i\right)
% \end{align}

